Interactive World Simulation with Cosmos for Physical AI

We present a shared framework that adapts Cosmos world foundation models for real-time interactive world simulation in Physical AI. By streaming visual observations in response to actions and scene controls, the framework enables users and embodied agents to interact with evolving virtual environments. It supports both predicting the visual consequences of actions and generating observations from physical state maintained by an external simulator. We demonstrate this approach across camera navigation and robot manipulation, controllable video transfer, and multi-view autonomous vehicle (AV) simulation. These examples provide a shared foundation for developing interactive virtual environments for Physical AI training and evaluation. Our code and model checkpoints are available at https://github.com/nvidia/cosmos and https://huggingface.co/collections/nvidia/cosmos3-examples. The project website is available at https://research.nvidia.com/labs/cosmos-lab/cosmos-simulation.

==> figures/bimanual/bimanual_robot_comparison/figure.tex <==
%
\providecommand{\CosmosFigureAssets}{images}%
\definecolor{cosmospath}{HTML}{3976A0}%
\definecolor{cosmosfuture}{HTML}{CBD7D3}%
\definecolor{cosmoscamera}{HTML}{D56829}%
\begin{tikzpicture}[x=1cm,y=-1cm]
\path[use as bounding box] (0,0) rectangle (16.24,7.38);
\begin{scope}
\clip (0,0) rectangle (3.2,1.8);
\fill[black!3] (0,0) rectangle (3.2,1.8);
\node[anchor=center,inner sep=0,outer sep=0] at (1.6,0.9) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0001.jpg}};
\end{scope}
\node[anchor=north west,inner sep=2pt,fill=black!60,fill opacity=.85,text opacity=1,text=white,font=\normalfont\bfseries\scriptsize] at (0.06,0.06) {Ground truth};
\begin{scope}
\clip (3.26,0) rectangle (6.46,1.8);
\fill[black!3] (3.26,0) rectangle (6.46,1.8);
\node[anchor=center,inner sep=0,outer sep=0] at (4.86,0.9) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0002.jpg}};
\end{scope}
\begin{scope}
\clip (6.52,0) rectangle (9.72,1.8);
\fill[black!3] (6.52,0) rectangle (9.72,1.8);
\node[anchor=center,inner sep=0,outer sep=0] at (8.12,0.9) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0003.jpg}};
\end{scope}
\begin{scope}
\clip (9.78,0) rectangle (12.98,1.8);
\fill[black!3] (9.78,0) rectangle (12.98,1.8);
\node[anchor=center,inner sep=0,outer sep=0] at (11.38,0.9) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0004.jpg}};
\end{scope}
\begin{scope}
\clip (13.04,0) rectangle (16.24,1.8);
\fill[black!3] (13.04,0) rectangle (16.24,1.8);
\node[anchor=center,inner sep=0,outer sep=0] at (14.64,0.9) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0005.jpg}};
\end{scope}
\begin{scope}
\clip (0,1.86) rectangle (3.2,3.66);
\fill[black!3] (0,1.86) rectangle (3.2,3.66);
\node[anchor=center,inner sep=0,outer sep=0] at (1.6,2.76) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0006.jpg}};
\end{scope}
\node[anchor=north west,inner sep=2pt,fill=black!60,fill opacity=.85,text opacity=1,text=white,font=\normalfont\bfseries\scriptsize] at (0.06,1.92) {DreamDojo 2B};
\begin{scope}
\clip (3.26,1.86) rectangle (6.46,3.66);
\fill[black!3] (3.26,1.86) rectangle (6.46,3.66);
\node[anchor=center,inner sep=0,outer sep=0] at (4.86,2.76) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0007.jpg}};
\end{scope}
\begin{scope}
\clip (6.52,1.86) rectangle (9.72,3.66);
\fill[black!3] (6.52,1.86) rectangle (9.72,3.66);
\node[anchor=center,inner sep=0,outer sep=0] at (8.12,2.76) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0008.jpg}};
\end{scope}
\begin{scope}
\clip (9.78,1.86) rectangle (12.98,3.66);
\fill[black!3] (9.78,1.86) rectangle (12.98,3.66);
\node[anchor=center,inner sep=0,outer sep=0] at (11.38,2.76) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0009.jpg}};
\end{scope}
\begin{scope}
\clip (13.04,1.86) rectangle (16.24,3.66);
\fill[black!3] (13.04,1.86) rectangle (16.24,3.66);
\node[anchor=center,inner sep=0,outer sep=0] at (14.64,2.76) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0010.jpg}};
\end{scope}
\begin{scope}
\clip (0,3.72) rectangle (3.2,5.52);
\fill[black!3] (0,3.72) rectangle (3.2,5.52);
\node[anchor=center,inner sep=0,outer sep=0] at (1.6,4.62) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0011.jpg}};
\end{scope}
\node[anchor=north west,inner sep=2pt,fill=black!60,fill opacity=.85,text opacity=1,text=white,font=\normalfont\bfseries\scriptsize] at (0.06,3.78) {DreamDojo 14B};
\begin{scope}
\clip (3.26,3.72) rectangle (6.46,5.52);
\fill[black!3] (3.26,3.72) rectangle (6.46,5.52);
\node[anchor=center,inner sep=0,outer sep=0] at (4.86,4.62) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0012.jpg}};
\end{scope}
\begin{scope}
\clip (6.52,3.72) rectangle (9.72,5.52);
\fill[black!3] (6.52,3.72) rectangle (9.72,5.52);
\node[anchor=center,inner sep=0,outer sep=0] at (8.12,4.62) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0013.jpg}};
\end{scope}
\begin{scope}
\clip (9.78,3.72) rectangle (12.98,5.52);
\fill[black!3] (9.78,3.72) rectangle (12.98,5.52);
\node[anchor=center,inner sep=0,outer sep=0] at (11.38,4.62) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0014.jpg}};
\end{scope}
\begin{scope}
\clip (13.04,3.72) rectangle (16.24,5.52);
\fill[black!3] (13.04,3.72) rectangle (16.24,5.52);
\node[anchor=center,inner sep=0,outer sep=0] at (14.64,4.62) {\includegraphics[width=3.2cm,height=1.8cm]{figures/bimanual/bimanual_robot_comparison/frame-0015.jpg}};
\end{scope}
\begin{scope}
\clip (0,5.58) rectangle (3.2,7.38);
\fill[black!3] (0,5.58) rectangle (3.2,7.38);
\node[anchor=center,inner sep=0,outer sep=0] at (1.6,6.48) {\includegraphics[width=3.2cm,height=1.76cm]{figures/bimanual/bimanual_robot_comparison/frame-0016.jpg}};
\end{scope}
\node[anchor=north west,inner sep=2pt,fill=black!60,fill opacity=.85,text opacity=1,text=white,font=\normalfont\bfseries\scriptsize] at (0.06,5.64) {Ours};
\begin{scope}
\clip (3.26,5.58) rectangle (6.46,7.38);
\fill[black!3] (3.26,5.58) rectangle (6.46,7.38);
\node[anchor=center,inner sep=0,outer sep=0] at (4.86,6.48) {\includegraphics[width=3.2cm,height=1.76cm]{figures/bimanual/bimanual_robot_comparison/frame-0017.jpg}};
\end{scope}
\begin{scope}
\clip (6.52,5.58) rectangle (9.72,7.38);
\fill[black!3] (6.52,5.58) rectangle (9.72,7.38);
\node[anchor=center,inner sep=0,outer sep=0] at (8.12,6.48) {\includegraphics[width=3.2cm,height=1.76cm]{figures/bimanual/bimanual_robot_comparison/frame-0018.jpg}};
\end{scope}
\begin{scope}
\clip (9.78,5.58) rectangle (12.98,7.38);
\fill[black!3] (9.78,5.58) rectangle (12.98,7.38);
\node[anchor=center,inner sep=0,outer sep=0] at (11.38,6.48) {\includegraphics[width=3.2cm,height=1.76cm]{figures/bimanual/bimanual_robot_comparison/frame-0019.jpg}};
\end{scope}
\begin{scope}
\clip (13.04,5.58) rectangle (16.24,7.38);
\fill[black!3] (13.04,5.58) rectangle (16.24,7.38);
\node[anchor=center,inner sep=0,outer sep=0] at (14.64,6.48) {\includegraphics[width=3.2cm,height=1.76cm]{figures/bimanual/bimanual_robot_comparison/frame-0020.jpg}};
\end{scope}
\end{tikzpicture}%


==> figures/diagrams/architecture_styles.tex <==
\setlength{\parfillskip}{0pt plus 1fil}
\definecolor{simtextfill}{HTML}{E0E0FF}
\definecolor{simtextedge}{HTML}{000073}
\definecolor{simcleanfill}{HTML}{D2E7F2}
\definecolor{simcleanedge}{HTML}{00476D}
\definecolor{simnoisyfill}{HTML}{FFF0E0}
\definecolor{simnoisyedge}{HTML}{C76300}
\definecolor{simactionfill}{HTML}{D9E7D7}
\definecolor{simactionedge}{HTML}{3D6039}
\definecolor{simgrayfill}{HTML}{ECECEC}
\definecolor{simgrayedge}{HTML}{4D4D4D}
\tikzset{
  sim token/.style={draw,minimum height=0.62cm,align=center,inner sep=2pt},
  sim text/.style={sim token,fill=simtextfill,draw=simtextedge},
  sim clean/.style={sim token,fill=simcleanfill,draw=simcleanedge},
  sim noisy/.style={sim token,fill=simnoisyfill,draw=simnoisyedge},
  sim action/.style={sim token,fill=simactionfill,draw=simactionedge},
  sim null/.style={sim token,fill=simgrayfill,draw=simgrayedge},
  sim stage/.style={draw=simgrayedge,rounded corners=2pt,align=center,
    minimum height=0.9cm,inner sep=5pt},
  sim flow/.style={->,semithick},
  sim grid/.style={draw=black!25,line width=0.25pt}
}


==> figures/diagrams/auto_camera_rig_geometry.tex <==
% Copyright (c) 2026 NVIDIA CORPORATION & AFFILIATES. All rights reserved.
% Symmetric schematic derived from Calibration setting A (retrieved 2026-10-22).
% Source: https://pages-f8576c.gitlab-master-pages.nvidia.com/camera-rig/example-rigs.js
% Source SHA-256: 87dfcedae895967a9604039eb7ba3811e3ced5584be4e5982c88088006f9e52a
% This is a schematic, not an exact calibration plot (explicit user request).
% Front/rear centers are on Y=0, with headings 0/180 degrees.
% Left/right pairs share mean longitudinal position and mean absolute Y.
% Cross/rear pairs use rounded mean absolute azimuth; side fisheyes use +/-90.
% FOV starts from the nearest degree, using the pair mean for paired cameras.
% The requested nominal display maps 119 to 120 degrees and 199/201 to 200.
% Sector boundaries use these displayed FOV values; source support is retained below.
% Circular horizontal sectors are centered on the schematic optical axes.
% Display radius: 4 m; neither occlusion nor sensing range is modeled.
% Paper coordinates (u,v) = (-Y,X), in meters; rear axle center is (0,0).
% Arrow lengths and numbered callout locations are display choices.

%
%
%
\expandafter\def\csname rigpos01\endcsname{(-0.000000,1.703462)}
\expandafter\def\csname rigaxis01\endcsname{(-0.000000,3.253462)}
\expandafter\def\csname rigfov01\endcsname{120}
\expandafter\def\csname rigpath01\endcsname{(-0.000000,1.703462) -- ++(30:4) arc[start angle=30,end angle=150,radius=4]}

%
%
%
\expandafter\def\csname rigpos02\endcsname{(0.913097,2.284898)}
\expandafter\def\csname rigaxis02\endcsname{(2.570006,2.988214)}
\expandafter\def\csname rigfov02\endcsname{120}
\expandafter\def\csname rigpath02\endcsname{(0.913097,2.284898) -- ++(-37:4) arc[start angle=-37,end angle=83,radius=4]}

%
%
%
\expandafter\def\csname rigpos03\endcsname{(0.968501,1.866876)}
\expandafter\def\csname rigaxis03\endcsname{(1.785684,0.263064)}
\expandafter\def\csname rigfov03\endcsname{70}
\expandafter\def\csname rigpath03\endcsname{(0.968501,1.866876) -- ++(-98:4) arc[start angle=-98,end angle=-28,radius=4]}

%
%
%
\expandafter\def\csname rigpos04\endcsname{(-0.000000,0.276583)}
\expandafter\def\csname rigaxis04\endcsname{(-0.000000,-1.523417)}
\expandafter\def\csname rigfov04\endcsname{30}
\expandafter\def\csname rigpath04\endcsname{(-0.000000,0.276583) -- ++(255:4) arc[start angle=255,end angle=285,radius=4]}

%
%
%
\expandafter\def\csname rigpos05\endcsname{(-0.968501,1.866876)}
\expandafter\def\csname rigaxis05\endcsname{(-1.785684,0.263064)}
\expandafter\def\csname rigfov05\endcsname{70}
\expandafter\def\csname rigpath05\endcsname{(-0.968501,1.866876) -- ++(208:4) arc[start angle=208,end angle=278,radius=4]}

%
%
%
\expandafter\def\csname rigpos06\endcsname{(-0.913097,2.284898)}
\expandafter\def\csname rigaxis06\endcsname{(-2.570006,2.988214)}
\expandafter\def\csname rigfov06\endcsname{120}
\expandafter\def\csname rigpath06\endcsname{(-0.913097,2.284898) -- ++(97:4) arc[start angle=97,end angle=217,radius=4]}

%
%
%
\expandafter\def\csname rigpos07\endcsname{(-0.000000,1.679798)}
\expandafter\def\csname rigaxis07\endcsname{(-0.000000,4.579798)}
\expandafter\def\csname rigfov07\endcsname{30}
\expandafter\def\csname rigpath07\endcsname{(-0.000000,1.679798) -- ++(75:4) arc[start angle=75,end angle=105,radius=4]}

%
%
%
\expandafter\def\csname rigpos08\endcsname{(-0.000000,3.680022)}
\expandafter\def\csname rigaxis08\endcsname{(-0.000000,5.480022)}
\expandafter\def\csname rigfov08\endcsname{200}
\expandafter\def\csname rigpath08\endcsname{(-0.000000,3.680022) -- ++(-10:4) arc[start angle=-10,end angle=190,radius=4]}

%
%
%
\expandafter\def\csname rigpos09\endcsname{(-0.989482,1.847646)}
\expandafter\def\csname rigaxis09\endcsname{(-2.789482,1.847646)}
\expandafter\def\csname rigfov09\endcsname{200}
\expandafter\def\csname rigpath09\endcsname{(-0.989482,1.847646) -- ++(80:4) arc[start angle=80,end angle=280,radius=4]}

%
%
%
\expandafter\def\csname rigpos10\endcsname{(0.989482,1.847646)}
\expandafter\def\csname rigaxis10\endcsname{(2.789482,1.847646)}
\expandafter\def\csname rigfov10\endcsname{200}
\expandafter\def\csname rigpath10\endcsname{(0.989482,1.847646) -- ++(-100:4) arc[start angle=-100,end angle=100,radius=4]}

%
%
%
\expandafter\def\csname rigpos11\endcsname{(-0.000000,-1.023335)}
\expandafter\def\csname rigaxis11\endcsname{(-0.000000,-2.823335)}
\expandafter\def\csname rigfov11\endcsname{196}
\expandafter\def\csname rigpath11\endcsname{(-0.000000,-1.023335) -- ++(172:4) arc[start angle=172,end angle=368,radius=4]}


==> figures/diagrams/auto_wsm_arrow_shapes.tex <==
%
%
%
\tikzset{wsm arrow forward/.pic={%
  \fill[wsmmarkingarrow]
    (-0.20000000,-0.50000000) -- (0.20000000,-0.50000000) -- (0.20000000,0.07600000) -- (0.50000000,0.07600000) --
    (0.00000000,0.50000000) -- (-0.50000000,0.07600000) -- (-0.20000000,0.07600000) -- cycle;
}}
\tikzset{wsm arrow left/.pic={%
  \fill[wsmmarkingarrow]
    (0.49828962,0.36590352) -- (0.49258837,0.36672118) -- (-0.01710376,0.36672118) -- (-0.04561003,0.37244481) --
    (-0.06670468,0.38716271) -- (-0.07411631,0.40760425) -- (-0.07411631,0.49632052) -- (-0.07582668,0.50000000) --
    (-0.08038769,0.49836468) -- (-0.49657925,0.27964023) -- (-0.50000000,0.27677841) -- (-0.49657925,0.27432543) --
    (-0.08038769,0.05560098) -- (-0.07582668,0.05396566) -- (-0.07411631,0.05764513) -- (-0.07411631,0.14595258) --
    (-0.06670468,0.16639411) -- (-0.04561003,0.18152085) -- (-0.01710376,0.18683565) -- (0.19213227,0.18683565) --
    (0.22063854,0.18152085) -- (0.24116306,0.16639411) -- (0.24914481,0.14595258) -- (0.24914481,-0.49427637) --
    (0.25028506,-0.49877351) -- (0.25655644,-0.50000000) -- (0.49258837,-0.50000000) -- (0.49828962,-0.49877351) --
    (0.50000000,-0.49427637) -- (0.50000000,0.36140638) -- cycle;
}}
\tikzset{wsm arrow right/.pic={%
  \fill[wsmmarkingarrow]
    (-0.49828962,0.36590352) -- (-0.49258837,0.36672118) -- (0.01710376,0.36672118) -- (0.04561003,0.37244481) --
    (0.06670468,0.38716271) -- (0.07411631,0.40760425) -- (0.07411631,0.49632052) -- (0.07582668,0.50000000) --
    (0.08038769,0.49836468) -- (0.49657925,0.27964023) -- (0.50000000,0.27677841) -- (0.49657925,0.27432543) --
    (0.08038769,0.05560098) -- (0.07582668,0.05396566) -- (0.07411631,0.05764513) -- (0.07411631,0.14595258) --
    (0.06670468,0.16639411) -- (0.04561003,0.18152085) -- (0.01710376,0.18683565) -- (-0.19213227,0.18683565) --
    (-0.22063854,0.18152085) -- (-0.24116306,0.16639411) -- (-0.24914481,0.14595258) -- (-0.24914481,-0.49427637) --
    (-0.25028506,-0.49877351) -- (-0.25655644,-0.50000000) -- (-0.49258837,-0.50000000) -- (-0.49828962,-0.49877351) --
    (-0.50000000,-0.49427637) -- (-0.50000000,0.36140638) -- cycle;
}}
\tikzset{wsm arrow left_forward/.pic={%
  \fill[wsmmarkingarrow]
    (0.07923497,-0.50000000) -- (0.31967213,-0.50000000) -- (0.31967213,0.07600000) -- (0.50000000,0.07600000) --
    (0.19945355,0.50000000) -- (-0.10109290,0.07600000) -- (0.07923497,0.07600000) -- cycle;
  \fill[wsmmarkingarrow]
    (0.19945355,-0.23040000) -- (0.19945355,-0.08960000) -- (-0.03661202,-0.08960000) -- (-0.03661202,0.01600000) --
    (-0.50000000,-0.16000000) -- (-0.03661202,-0.33600000) -- (-0.03661202,-0.23040000) -- cycle;
}}
\tikzset{wsm arrow right_forward/.pic={%
  \fill[wsmmarkingarrow]
    (-0.31967213,-0.50000000) -- (-0.07923497,-0.50000000) -- (-0.07923497,0.07600000) -- (0.10109290,0.07600000) --
    (-0.19945355,0.50000000) -- (-0.50000000,0.07600000) -- (-0.31967213,0.07600000) -- cycle;
  \fill[wsmmarkingarrow]
    (-0.19945355,-0.08960000) -- (-0.19945355,-0.23040000) -- (0.03661202,-0.23040000) -- (0.03661202,-0.33600000) --
    (0.50000000,-0.16000000) -- (0.03661202,0.01600000) -- (0.03661202,-0.08960000) -- cycle;
}}
\tikzset{wsm arrow merge_left/.pic={%
  \fill[wsmmarkingarrow]
    (0.33823529,-0.50000000) -- (0.50000000,-0.33823529) -- (-0.02941176,0.19117647) -- (0.09191176,0.31250000) --
    (-0.50000000,0.50000000) -- (-0.31250000,-0.09191176) -- (-0.19117647,0.02941176) -- cycle;
}}
\tikzset{wsm arrow merge_right/.pic={%
  \fill[wsmmarkingarrow]
    (-0.50000000,-0.33823529) -- (-0.33823529,-0.50000000) -- (0.19117647,0.02941176) -- (0.31250000,-0.09191176) --
    (0.50000000,0.50000000) -- (-0.09191176,0.31250000) -- (0.02941176,0.19117647) -- cycle;
}}


==> figures/diagrams/auto_wsm_styles.tex <==
%
%
\input{figures/diagrams/architecture_styles.tex}
\definecolor{wsmsignstop}{RGB}{220,20,20}
\definecolor{wsmsignyield}{RGB}{255,140,0}
\definecolor{wsmsigndonotenter}{RGB}{200,0,100}
\definecolor{wsmsignoneway}{RGB}{40,110,220}
\definecolor{wsmsignleft}{RGB}{0,180,230}
\definecolor{wsmsignright}{RGB}{30,60,200}
\definecolor{wsmsignpedestrian}{RGB}{255,220,0}
\definecolor{wsmsignother}{RGB}{8,2,255}
\definecolor{wsmsignback}{RGB}{40,40,40}
\definecolor{wsmlightred}{RGB}{240,50,50}
\definecolor{wsmlightyellow}{RGB}{255,200,0}
\definecolor{wsmlightgreen}{RGB}{130,240,132}
\definecolor{wsmlightredyellow}{RGB}{208,136,72}
\definecolor{wsmlightwhite}{RGB}{255,255,255}
\definecolor{wsmlightunknown}{RGB}{150,150,150}
\definecolor{wsmlightoff}{RGB}{20,20,20}
\definecolor{wsmlighthousing}{RGB}{105,105,105}
\definecolor{wsmlightback}{RGB}{60,60,60}
\definecolor{wsmlightedge}{RGB}{200,200,200}
\definecolor{wsmmarkingarrow}{RGB}{244,244,244}
\definecolor{wsmmarkingstop}{RGB}{255,0,0}
\definecolor{wsmmarkingclear}{RGB}{0,255,32}
\definecolor{wsmmarkingother}{RGB}{20,254,185}
\definecolor{wsmboundarybarrier}{RGB}{253,1,232}
\definecolor{wsmboundarycurb}{RGB}{207,255,191}
\definecolor{wsmboundaryseam}{RGB}{0,159,96}
\definecolor{wsmboundaryposts}{RGB}{255,207,159}
\definecolor{wsmboundarywall}{RGB}{0,128,159}
\definecolor{wsmboundaryother}{RGB}{239,191,255}

\tikzset{
  wsm chart/.style={font=\fontfamily{bch}\fontsize{9}{11}\selectfont},
  wsm title/.style={font=\fontfamily{bch}\fontsize{10}{12}\selectfont\bfseries,
    anchor=west,inner sep=0pt},
  wsm label/.style={font=\fontfamily{bch}\fontsize{9}{11}\selectfont\bfseries},
  wsm values/.style={font=\fontfamily{bch}\fontsize{8}{10}\selectfont},
  wsm note/.style={font=\fontfamily{bch}\fontsize{8}{10}\selectfont,
    align=left,anchor=west,inner sep=0pt},
  wsm card/.style={draw=simgrayedge!45,line width=0.35pt,rounded corners=2pt},
  wsm rule/.style={draw=simgrayedge!35,line width=0.3pt}
}

%
\newcommand{\wsmhex}[1]{\convertcolorspec{named}{#1}{HTML}\wsmvalue\#\wsmvalue}
\newcommand{\wsmrgb}[1]{\convertcolorspec{named}{#1}{RGB}\wsmvalue(\wsmvalue)}
\newcommand{\wsmcolorspec}[1]{\wsmhex{#1}\quad RGB\,\wsmrgb{#1}}

%
\newcommand{\wsmlightface}[3]{%
  \begin{scope}[shift={(#1,#2)},x=0.72cm,y=0.72cm]
    \fill[wsmlighthousing] (-0.5,-0.5) rectangle (0.5,0.5);
    #3
    \draw[wsmlightedge,line width=0.45pt] (-0.5,-0.5) rectangle (0.5,0.5);
  \end{scope}}
\newcommand{\wsmring}[1]{%
  %
  %
  \fill[#1,even odd rule]
    plot[domain=0:360,samples=25,variable=\wsmangle]
      ({0.46*cos(\wsmangle)},{0.46*sin(\wsmangle)}) -- cycle
    plot[domain=0:360,samples=25,variable=\wsmangle]
      ({0.30*cos(\wsmangle)},{0.30*sin(\wsmangle)}) -- cycle;}
\newcommand{\wsmcross}{%
  %
  \pgfmathsetmacro{\wsminset}{0.15*sqrt(2)}
  \fill[wsmlightred] (-0.5,{-0.5+\wsminset}) -- ({-0.5+\wsminset},-0.5)
    -- (0.5,{0.5-\wsminset}) -- ({0.5-\wsminset},0.5) -- cycle;
  \fill[wsmlightred] (-0.5,{0.5-\wsminset}) -- ({-0.5+\wsminset},0.5)
    -- (0.5,{-0.5+\wsminset}) -- ({0.5-\wsminset},-0.5) -- cycle;}


==> figures/introduction/icons/nvidia_icons.tex <==
%
%
%
\usetikzlibrary{svg.path}
\tikzset{
  %
  pics/overview manipulation/.style={code={
    \begin{scope}[shift={(-0.55cm,0.55cm)}]
      \begin{scope}[xscale=0.6520423228,yscale=-0.6520423228]
        \path[fill=simactionedge,draw=none] svg {M 35.974 23.5 L 37.5 29.27 L 37.5 40.5 L 36.5 40.5 L 36.5 34.5 L 32.5 34.5 L 32.5 40.5 L 31.5 40.5 L 31.5 24.5 L 16.5 24.5 L 16.501 40.5 L 15.502 40.5 L 15.501 34.5 L 11.5 34.5 L 11.5 40.5 L 10.5 40.5 L 10.509 34.5 L 10.5 34.5 L 10.5 33.5 L 10.51 33.5 L 10.517 29.141 L 12.026 23.5 L 20.5 23.5 L 20.5 21.5 L 19.686 21.5 L 18.632 17.5 L 16.5 17.5 L 16.5 10.5 L 18.5 10.5 L 18.5 9.793 L 20.793 7.5 L 27.207 7.5 L 29.5 9.793 L 29.498 10.5 L 31.5 10.5 L 31.5 17.5 L 29.384 17.5 L 28.313 21.5 L 27.5 21.5 L 27.5 23.5 Z M 19.5 16.935 L 20.454 20.5 L 27.546 20.5 L 28.5 16.934 L 28.5 10.207 L 26.793 8.5 L 21.207 8.5 L 19.5 10.207 Z M 11.5 33.5 L 15.501 33.5 L 15.5 24.5 L 12.794 24.5 L 11.5 29.336 Z M 32.5 24.5 L 32.5 33.5 L 36.5 33.5 L 36.5 29.336 L 35.206 24.5 Z M 21.5 21.5 L 21.5 23.5 L 26.5 23.5 L 26.5 21.5 Z M 18.5 11.5 L 17.5 11.5 L 17.5 16.5 L 18.5 16.5 Z M 30.5 11.5 L 29.5 11.5 L 29.5 16.5 L 30.5 16.5 Z};
        \path[fill=simactionedge,draw=none] svg {M 29.5 31.5 L 18.5 31.5 L 18.5 26.5 L 29.5 26.5 Z M 28.5 27.5 L 19.5 27.5 L 19.5 30.5 L 28.5 30.5 Z};
      \end{scope}
    \end{scope}
  }},
  %
  pics/overview transfer/.style={code={
    \begin{scope}[shift={(-0.55cm,0.55cm)}]
      \begin{scope}[xscale=0.6520423228,yscale=-0.6520423228]
        \path[fill=simactionedge,draw=none] svg {M 40.5 7.5 L 40.5 8.5 L 7.5 8.5 L 7.5 7.5 Z M 7.5 16.5 L 40.5 16.5 L 40.5 15.5 L 7.5 15.5 Z M 37.5 14.5 L 40.5 14.5 L 40.5 13.5 L 38.5 13.5 L 38.5 10.5 L 40.5 10.5 L 40.5 9.5 L 37.5 9.5 Z M 10.5 9.5 L 7.5 9.5 L 7.5 10.5 L 9.5 10.5 L 9.5 13.5 L 7.5 13.5 L 7.5 14.5 L 10.5 14.5 Z M 18.5 9.5 L 18.5 14.5 L 13.5 14.5 L 13.5 9.5 Z M 17.5 10.5 L 14.5 10.5 L 14.5 13.5 L 17.5 13.5 Z M 26.5 9.5 L 26.5 14.5 L 21.5 14.5 L 21.5 9.5 Z M 25.5 10.5 L 22.5 10.5 L 22.5 13.5 L 25.5 13.5 Z M 34.5 9.5 L 34.5 14.5 L 29.5 14.5 L 29.5 9.5 Z M 33.5 10.5 L 30.5 10.5 L 30.5 13.5 L 33.5 13.5 Z M 7.5 32.5 L 40.5 32.5 L 40.5 31.5 L 7.5 31.5 Z M 7.5 40.5 L 40.5 40.5 L 40.5 39.5 L 7.5 39.5 Z M 37.5 38.5 L 40.5 38.5 L 40.5 37.5 L 38.5 37.5 L 38.5 34.5 L 40.5 34.5 L 40.5 33.5 L 37.5 33.5 Z M 10.5 33.5 L 7.5 33.5 L 7.5 34.5 L 9.5 34.5 L 9.5 37.5 L 7.5 37.5 L 7.5 38.5 L 10.5 38.5 Z M 18.5 33.5 L 18.5 38.5 L 13.5 38.5 L 13.5 33.5 Z M 17.5 34.5 L 14.5 34.5 L 14.5 37.5 L 17.5 37.5 Z M 26.5 33.5 L 26.5 38.5 L 21.5 38.5 L 21.5 33.5 Z M 25.5 34.5 L 22.5 34.5 L 22.5 37.5 L 25.5 37.5 Z M 34.5 33.5 L 34.5 38.5 L 29.5 38.5 L 29.5 33.5 Z M 33.5 34.5 L 30.5 34.5 L 30.5 37.5 L 33.5 37.5 Z M 29.5 19.5 L 28.5 19.5 L 28.5 26.5 L 27.5 26.5 L 27.5 27.5 L 28.5 27.5 L 28.5 28.5 L 29.5 28.5 L 29.5 27.5 L 30.5 27.5 L 30.5 26.5 L 29.5 26.5 Z M 34.5 19.5 L 33.5 19.5 L 33.5 20.5 L 32.5 20.5 L 32.5 21.5 L 33.5 21.5 L 33.5 28.5 L 34.5 28.5 L 34.5 21.5 L 35.5 21.5 L 35.5 20.5 L 34.5 20.5 Z M 24.5 19.5 L 23.5 19.5 L 23.5 23.5 L 22.5 23.5 L 22.5 24.5 L 23.5 24.5 L 23.5 28.5 L 24.5 28.5 L 24.5 24.5 L 25.5 24.5 L 25.5 23.5 L 24.5 23.5 Z M 19.5 19.5 L 18.5 19.5 L 18.5 20.5 L 17.5 20.5 L 17.5 21.5 L 18.5 21.5 L 18.5 28.5 L 19.5 28.5 L 19.5 21.5 L 20.5 21.5 L 20.5 20.5 L 19.5 20.5 Z M 14.5 19.5 L 13.5 19.5 L 13.5 26.5 L 12.5 26.5 L 12.5 27.5 L 13.5 27.5 L 13.5 28.5 L 14.5 28.5 L 14.5 27.5 L 15.5 27.5 L 15.5 26.5 L 14.5 26.5 Z M 7.5 17.5 L 40.5 17.5 L 40.5 30.5 L 7.5 30.5 Z M 8.5 29.5 L 39.5 29.5 L 39.5 18.5 L 8.5 18.5 Z};
      \end{scope}
    \end{scope}
  }},
  %
  pics/overview av/.style={code={
    \begin{scope}[shift={(-0.55cm,0.55cm)}]
      \begin{scope}[xscale=0.6520423228,yscale=-0.6520423228]
        \path[fill=simactionedge,draw=none] svg {M 36.5 30.5 L 11.5 30.5 L 11.5 31.5 L 36.5 31.5 Z M 16.2 24.5 L 31.8 24.5 L 32.8 23.5 L 38.5 23.5 L 38.5 25 C 38.5 26.9 36.9 28.5 35 28.5 L 13 28.5 C 11.1 28.5 9.5 26.9 9.5 25 L 9.5 23.5 L 15.2 23.5 Z M 37.5 25 L 37.5 24.5 L 33.2 24.5 L 32.2 25.5 L 15.8 25.5 L 14.8 24.5 L 10.5 24.5 L 10.5 25 C 10.5 26.4 11.6 27.5 13 27.5 L 35 27.5 C 36.4 27.5 37.5 26.4 37.5 25};
        \path[fill=simactionedge,draw=none] svg {M 39.2 20.5 C 40.6 21.5 41.5 23.1 41.5 25 L 41.5 35.7 C 41.5 36.7 40.7 37.5 39.8 37.5 L 36.2 37.5 C 35.3 37.5 34.5 36.7 34.5 35.7 L 34.5 33.5 L 13.5 33.5 L 13.5 35.5 C 13.5 36.6 12.7 37.5 11.8 37.5 L 8.2 37.5 C 7.3 37.5 6.5 36.6 6.5 35.5 L 6.5 25 C 6.5 23.1 7.4 21.5 8.8 20.5 L 5.3 20.5 L 6.1 17.5 L 10.4 17.5 L 11.3 14.5 C 12 12.1 14.2 10.5 16.6 10.5 L 31.4 10.5 C 33.9 10.5 36 12.2 36.7 14.5 L 37.6 17.5 L 41.9 17.5 L 42.7 20.5 Z M 40.5 32.5 L 40.5 25 C 40.5 22.5 38.5 20.5 36 20.5 L 12 20.5 C 9.5 20.5 7.5 22.5 7.5 25 L 7.5 32.5 Z M 12.3 14.8 L 11 19.5 L 36.9 19.5 L 36.6 18.5 L 36.6 18.4 L 35.6 14.8 C 35.1 12.8 33.3 11.5 31.3 11.5 L 16.6 11.5 C 14.6 11.5 12.8 12.9 12.3 14.8 M 40.5 35.7 L 40.5 33.5 L 35.5 33.5 L 35.5 35.7 C 35.5 36.1 35.8 36.5 36.2 36.5 L 39.8 36.5 C 40.2 36.5 40.5 36.2 40.5 35.7 M 12.5 35.5 L 12.5 33.5 L 7.5 33.5 L 7.5 35.5 C 7.5 36 7.8 36.5 8.2 36.5 L 11.8 36.5 C 12.2 36.5 12.5 36 12.5 35.5 M 41.1 18.5 L 37.8 18.5 L 38.1 19.5 L 41.4 19.5 Z M 6.9 18.5 L 6.6 19.5 L 9.9 19.5 L 10.2 18.5 Z};
      \end{scope}
    \end{scope}
  }},
}


==> figures/latency/latency_bimanual_compiled_stages_data.tex <==
%
%
%
\newcommand{\bimanuallatencyrowcount}{1}
\newcommand{\bimanuallatencyrows}{%
  \bimanuallatencyrow{0}{compiled + CUDA graphs}{88.551826513139531}{69.178434991044924}{4.4099998474121094}{4.6965930541045964}{167}%
}


==> figures/latency/latency_bimanual_stages.tex <==
%
%
\begingroup
\input{figures/diagrams/architecture_styles.tex}

  \input{figures/latency/latency_bimanual_compiled_stages_data.tex}
  \def\latencyxunit{0.058cm}
  \def\latencylabelwidth{3.5cm}
  \def\latencytickstep{20}
  \def\latencyticklast{160}
  \def\latencyxmax{180}

\pgfmathsetmacro{\latencybottom}{-0.70*(\bimanuallatencyrowcount-1)-0.40}

\newcommand{\bimanuallatencyrow}[7]{%
  \pgfmathsetmacro{\rowy}{-0.70*#1}
  \node[anchor=east,align=right,inner sep=0pt,xshift=-5pt] at (0,\rowy) {#2};
  \foreach \duration/\stage [remember=\stageright as \stageleft (initially 0)]
    in {#3/denoise,#4/cache,#5/decode,#6/other} {
    \pgfmathsetmacro{\stageright}{\stageleft+\duration}
    \ifdim\duration pt>0pt
      \path[latency \stage] (\stageleft,{\rowy-0.18}) rectangle (\stageright,{\rowy+0.18});
    \fi
  }
  \pgfmathsetmacro{\stagetotal}{#3+#4+#5+#6}
  \node[anchor=west,inner sep=0pt,xshift=3pt] at (\stagetotal,\rowy) {#7};
}
\fitdiagram{%
\begin{tikzpicture}[x=1cm,y=1cm,
  font=\fontfamily{bch}\fontsize{8}{9.5}\selectfont,
  every node/.append style={text=.},
  latency denoise/.style={fill=simnoisyfill,draw=simnoisyedge,line width=0.4pt},
  latency cache/.style={fill=simcleanfill,draw=simcleanedge,line width=0.4pt},
  latency decode/.style={fill=simgrayfill,draw=simgrayedge,line width=0.4pt},
  latency other/.style={fill=white,draw=simgrayedge,line width=0.4pt}]
  \node[anchor=west,inner sep=0pt,
    font=\fontfamily{bch}\fontsize{9}{10.5}\selectfont\bfseries] at (0,0.65)
    {Cosmos3-Nano-Sim-Bimanual, one GB300};
  \begin{scope}[xshift=\latencylabelwidth,x=\latencyxunit]
    \foreach \tick in {0,\latencytickstep,...,\latencyticklast} {
      \draw[simgrayedge!20,line width=0.3pt] (\tick,0.28) -- (\tick,\latencybottom);
      \node[anchor=north,inner sep=2pt] at (\tick,\latencybottom) {\tick};
    }
    \draw[simgrayedge!65,line width=0.4pt] (0,\latencybottom) -- (\latencyxmax,\latencybottom);
    \bimanuallatencyrows
    \node[anchor=north,inner sep=0pt] at ({\latencyxmax/2},{\latencybottom-0.45})
      {Per-chunk time (ms), p50 over steady-state chunks};
  \end{scope}
  \foreach \x/\stage/\label in {
    2.0/denoise/Denoise,
    4.5/cache/{K/V cache update},
    8.5/decode/Decode,
    11.0/other/Other} {
    \path[latency \stage] (\x,{\latencybottom-1.18}) rectangle ++(0.35,0.23);
    \node[anchor=west,inner sep=0pt] at ({\x+0.48},{\latencybottom-1.065}) {\label};
  }
\end{tikzpicture}}
\endgroup

